On the Soundness of Infrastructure Adversaries

Companies and network operators perform risk assessment to inform policy-making, guide infrastructure investments or to comply with security standards such as ISO 27001. Due to the size and complexity of these networks, risk assessment techniques such as attack graphs or trees describe the attacker with a finite set of rules. This characterization of the attacker can easily miss attack vectors or overstate them, potentially leading to incorrect risk estimation. In this work, we propose the first methodology to justify a rule-based attacker model. Conceptually, we add another layer of abstraction on top of the symbolic model of cryptography, which reasons about protocols and abstracts cryptographic primitives. This new layer reasons about Internet-scale networks and abstracts protocols. We show, in general, how the soundness and completeness of a rule-based model can be ensured by verifying trace properties, linking soundness to safety properties and completeness to liveness properties. We then demonstrate the approach for a recently proposed threat model that quantifies the confidentiality of email communication on the Internet, including DNS, DNSSEC, and SMTP. Using off-the-shelf protocol verification tools, we discover two flaws in their threat model. After fixing them, we show that it provides symbolic soundness.

==> infra_attacker_motivation.tex <==
\section{Motivation}
% Problem Statement
The internet infrastructure describes an extensive network 
of networks used by billions of users a day. Such a vast 
infrastructure heavily depends on the correct functionality 
of the underlying protocols in its layered structure (e.g., 
Ethernet, IP, TCP, DNS).
%

However, the Internet was developed with functionality and 
not security in mind. For decades the security 
research-community contributed lots of mechanisms, protocols 
(and extensions of existing ones) as well as entirely new 
concepts to secure the infrastructure post-hoc. Security of 
infrastructures and networks is still (and more than ever) 
an ongoing research effort with several open problems and 
research questions.
%



% Approaches to secure the infrastructure and analyze it
Preventing exploits on infrastructure level needs mechanisms 
to detect potential risks on the hand and strategies to design 
networks securely by construction. While the latter could be 
the way to go for new infrastructures, it is undoubtedly hard 
in already existing ones like the Internet. Hence, detecting 
and fixing design flaws in huge networks is an ongoing research 
effort. 
%

%Several approaches in analyzing networks have been studied, 
%attempting to get some methodology in finding vulnerabilities. 
%Graph-based approaches were used to model the infrastructure 
%using attack graphs \citep{swiler1998graph}, labeled property 
%graphs \citep{cispa1091} or to enable intrusion detection using 
%activity graphs \citep{staniford1996grids}. Also, formal methods 
%were used to base infrastructure security on a model checking 
%approach \citep{ritchey2000using}.

% Large scale look at Economical Approach
%Further, there were recent approaches in performing deployment 
%assessment of security mechanisms in vast networks 
%\cite{speicher2018formally}. In this approach, they analyze 
%networks using an attacker/ defender scenario utilizing Stackelberg 
%planning \citep{speicher2018stackelberg}.
%
%Using the property graph model by \citep{cispa1091}, they 
%introduced the first methodology for large-scale formal deployment 
%assessments in the case of email infrastructure. Their work 
%introduces a rule-based threat model (see Section6) based on 
%formally proven security and trust assumptions of security 
%protocols. This threat model features a finite set of rules 
%allowing for efficient analysis even in massive networks. However, 
%justification of that threat model is still an open problem that we 
%aim to cope with this work.


% Transition to other subsections
%First, we will take a more detailed look at the work of 
%\citep{speicher2018formally} by starting to provide the necessary background.
%In the following sections, we will then proceed by  justifying
%their threat models using formal methods.

==> lstsettings-apip.tex <==
\lstdefinelanguage{apip}{
  morekeywords=[1]{
    %%% KEYWORDS
	out, in, if, then, else, event, insert, delete, lookup, as, in, lock, unlock, let
    },
  sensitive=true,
  morecomment=[l]{\#},
  morecomment=[l]{//},
  morestring=[b]',
  morestring=[s]{`}{'},
  % morestring=[s]{[}{]},
}

\lstdefinestyle{apip}{
    language={apip}, 
	stringstyle=\rm\textup,
	keywordstyle=[1]\sf,
 	keywordstyle=[2]\rm\upshape,
	literate={||}{{$\mid$}}1
	{new}{{$\nu$}}1
	{<}{{$\langle$}}1
	{>}{{$\rangle$}}1
	{(}{{$($}}1
	{)}{{$)$}}1
}


\lstset{style=apip,
	mathescape=true, 
	commentstyle=\rm\itshape,
	showstringspaces=false,
    frameround=ftff,
    % frame=single,
	captionpos=b,
	columns=flexible,
escapeinside={(*}{*)},
basicstyle=\it\small,	
% escapechar=!,
tabsize=2,
breaklines=true,
showstringspaces=true,
emph={label}
} 

% vim: ft=tex

